MagicClay: Sculpting Meshes With Generative Neural Fields

The recent developments in neural fields have brought phenomenal capabilities to the field of shape generation, but they lack crucial properties, such as incremental control - a fundamental requirement for artistic work. Triangular meshes, on the other hand, are the representation of choice for most geometry related tasks, offering efficiency and intuitive control, but do not lend themselves to neural optimization. To support downstream tasks, previous art typically proposes a two-step approach, where first a shape is generated using neural fields, and then a mesh is extracted for further processing. Instead, in this paper we introduce a hybrid approach that maintains both a mesh and a Signed Distance Field (SDF) representations consistently. Using this representation, we introduce MagicClay - an artist friendly tool for sculpting regions of a mesh according to textual prompts while keeping other regions untouched. Our framework carefully and efficiently balances consistency between the representations and regularizations in every step of the shape optimization; Relying on the mesh representation, we show how to render the SDF at higher resolutions and faster. In addition, we employ recent work in differentiable mesh reconstruction to adaptively allocate triangles in the mesh where required, as indicated by the SDF. Using an implemented prototype, we demonstrate superior generated geometry compared to the state-of-the-art, and novel consistent control, allowing sequential prompt-based edits to the same mesh for the first time.

==> content/tables/quantitative_results_uncond_detailed_suppmat.tex <==

\begin{table*}[t]
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|}
 &  P1$\uparrow$ &  P2 $\uparrow$ &  P3 $\uparrow$ &  P4 $\uparrow$ &  P5 $\uparrow$ &  P6 $\uparrow$ &  P7 $\uparrow$ &  P8 $\uparrow$ &  P9 $\uparrow$ &  P10 $\uparrow$ & mean $\uparrow$ \\
 \hline
 Fantasia3D (Mesh) &  23.73&  22.62&  25.54&  20.06&  25.88&  22.69&  26.81&  22.47&  25.01&  24.84 &23.97
\\
 \hline
 ProlificDreamer (NeRF)&  22.22&  21.54&  22.51&  21.35& 22.87 &  21.8&  16.65&  20.26&  23.33& ?? &21.21
 \\
 
 ProlificDreamer (Mesh)& 22.82  & 20.11 & 19.46  & 20.89 & 20.94 & 21.53 & 14.4 & 19.7  & 21.6 & 19.46 & 20.06 \\
  \hline
 Hifa (NeRF) & 27.43 & 20.46 & 24.17 & 20.46 & 20.81 & 19.59 & 22.09 & 24.56 & 26.55  & 25.22 & 23.16 \\
 
 Hifa (Mesh) & 26.67 & 17.13 & 22.04 & 20.38 & 19.74 & 19.35 & 19.33 & 24.41 & 26.79  & 24.84 & 22.01 \\
\hline
 TextMesh (SDF) & 24.11 & 22.17 & 28.65 & 21.13  & 24.79 & 22.61 & 27.68 & 27.38 & 25.63 & 25.23 & 24.92 \\
  TextMesh (Mesh) & 28.69 & 20.0 & 25.23 & 20.52 & 21.54 & 21.56 & 23.86 & 24.53 & 24.09 & 22.59 & 23.56 \\
  \hline
   MVDreams (NeRF) & 25.42 & 25.29 & 23.39 & 25.34 & 25.14 & 26.08 & 27.51 &  & 24.98 & 26.67 & 25.43 \\
   MVDreams (Mesh) & 23.59 & 24.95 & 22.45 &  & 24.56 & 26.92 & 22.50 & 20.77 & 27.16 & 25.59 & 24.05 \\
  \hline
 ours (SDF) & 24.32 &  &  &  &  &  &  &  &  &  &  \\
ours (Mesh) & \textbf{30.7125} &  &  &  &  &  &  &  &  &  &  \\
  \hline
\end{tabular}
\caption{{\bf Quantitative comparison.} \todo{unconditional 3D generation}. We calculate the average clip score for 25 normal renders of the NeRFs/SDFs and meshes for various generative pipelines, taken in a equidistant circular pattern around the generated object. We apply marching cubes to extract the resulting meshes from the NeRFs/SDFs. There is a noticeable drop in the clip score for all single representation pipelines between the renders of the implicit function and the extracted mesh, which can qualitatively be seen in \ref{fig:gen_comparison}. \todo{keep only mean in main paper, put details in sup mat, use 20 prompts). We don't have the drop because we optimize the mesh part as well. Mention clip socre is cosine similarity} }
\end{table*}
